Statistical strong lensing. II. Cosmology and galaxy structure with time-delay lenses

Context. Time delay lensing is a powerful tool to measure the Hubble constant $H_0$. In order to obtain an accurate estimate of $H_0$ from a sample of time delay strong lenses, however, it is necessary to have a very good knowledge of the mass structure of the lens galaxies. Strong lensing data on their own are not sufficient to break the degeneracy between $H_0$ and the lens model parameters, on a single object basis. Aims. The goal of this study is to determine whether it is possible to break the $H_0$-lens structure degeneracy with the statistical combination of a large sample of time-delay lenses, relying purely on strong lensing data (that is, with no stellar kinematics information). Methods. I simulated a set of 100 lenses with doubly imaged quasars and related time delay measurements. I fitted these data with a Bayesian hierarchical method and a flexible model for the lens population, emulating the lens modelling step. Results. The sample of 100 lenses, on its own, provides a measurement of $H_0$ with $3\%$ precision, but with a $-4\%$ bias. However, the addition of prior information on the lens structural parameters from a large sample of lenses with no time delays, such as that considered in Paper I, allows for a $1\%$-level inference. Moreover, the 100 lenses allow for a $0.03$~dex calibration of galaxy stellar masses, regardless of the level of prior knowledge of the Hubble constant. Conclusions. Breaking the $H_0$-lens model degeneracy with lensing data alone is possible, but $1\%$ measurements of $H_0$ require either a number of time delay lenses much larger than 100, or the knowledge of the structural parameter distribution of the lens population from a separate sample of lenses.

==> h0_inference_table.tex <==
$H_0$ & $70$ & $U(50,90)$ & $67.5_{-2.2}^{+1.7}$ & $69.4_{-0.8}^{+0.8}$ & $69.6_{-0.6}^{+0.6}$ & Hubble constant, in km s$^{-1}$ Mpc$^{-1}$ \\
$\mu_{\mathrm{DM}, 0}$ & $11.04$ & $U(10,12)$ & $11.06_{-0.02}^{+0.03}$ & $11.052_{-0.008}^{+0.008}$ & $11.09_{-0.02}^{+0.02}$ & Mean $\log{\mfive}$ at $\log{\msps}=11.4$ and \\
 & & & & & & average size \\
$\beta_{\mathrm{DM}}$ & $0.57$ & $U(0,3)$ & $0.49_{-0.06}^{+0.06}$ & $0.56_{-0.02}^{+0.02}$ & $0.53_{-0.05}^{+0.06}$ & Dependence of $\log{\mfive}$ on $\msps$ \\
$\xi_{\mathrm{DM}}$ & $-0.15$ & $U(-1,1)$ & $-0.20_{-0.12}^{+0.10}$ & $-0.13_{-0.04}^{+0.04}$ & $-0.21_{-0.11}^{+0.09}$ & Dependence of $\log{\mfive}$ on galaxy size \\
$\sigma_{\mathrm{DM}}$ & $0.05$ & $U(0.0,0.5)$ & $0.032_{-0.009}^{+0.014}$ & $0.058_{-0.008}^{+0.008}$ & $0.035_{-0.011}^{+0.017}$ & Intrinsic scatter in $\log{\mfive}$ \\
$\mu_{\gamma,0}$ & $1.47$ & $U(0,1)$ & $1.38_{-0.12}^{+0.10}$ & $1.44_{-0.02}^{+0.02}$ & $1.48_{-0.06}^{+0.06}$ & Mean $\gammadm$ at $\log{\msps}=11.4$ and \\
 & & & & & & average size \\
$\beta_{\gamma}$ & $-0.39$ & $U(-1,1)$ & $-0.37_{-0.10}^{+0.10}$ & $-0.27_{-0.04}^{+0.04}$ & $-0.42_{-0.10}^{+0.10}$ & Dependence of $\gammadm$ on $\log{\msps}$ \\
$\xi_{\gamma}$ & $-0.37$ & $U(-1,1)$ & $-0.4_{-0.2}^{+0.2}$ & $-0.28_{-0.08}^{+0.08}$ & $-0.47_{-0.19}^{+0.18}$ & Dependence of $\gammadm$ on galaxy size \\
$\sigma_{\gamma}$ & $0.06$ & $U(0.0,0.5)$ & $0.08_{-0.04}^{+0.05}$ & $0.059_{-0.017}^{+0.016}$ & $0.07_{-0.03}^{+0.03}$ & Intrinsic scatter in $\gammadm$ \\
$\log{\alpha_{\mathrm{sps}}}$ & $0.10$ & $U(0.00,0.25)$ & $0.11_{-0.02}^{+0.02}$ & $0.101_{-0.007}^{+0.007}$ & $0.10_{-0.03}^{+0.02}$ & Log of the stellar population synthesis \\
 & & & & & & mismatch parameter \\

